Data Safety vs. App Privacy: Comparing the Usability of Android and iOS Privacy Labels

Privacy labels -- standardized, compact representations of data collection and data use practices -- are often presented as a solution to the shortcomings of privacy policies. Apple introduced mandatory privacy labels for apps in its App Store in December 2020; Google introduced mandatory labels for Android apps in July 2022. iOS app privacy labels have been evaluated and critiqued in prior work. In this work, we evaluated Android Data Safety Labels and explored how differences between the two label designs impact user comprehension and label utility. We conducted a between-subjects, semi-structured interview study with 12 Android users and 12 iOS users. While some users found Android Data Safety Labels informative and helpful, other users found them too vague. Compared to iOS App Privacy Labels, Android users found the distinction between data collection groups more intuitive and found explicit inclusion of omitted data collection groups more salient. However, some users expressed skepticism regarding elided information about collected data type categories. Most users missed critical information due to not expanding the accordion interface, and they were surprised by collection practices excluded from Android's definitions. Our findings also revealed that Android users generally appreciated information about security practices included in the labels, and iOS users wanted that information added.

==> figures/freq_terminology.tex <==

\begin{figure}
    %\centering
    \caption{Terminology used to present relative frequency of themes}
    \label{fig:freq_term}
     \begin{tikzpicture}[snake=zigzag, line before snake = 5mm, line after snake = 5mm]
    % draw horizontal line 
    \draw[thick,<-] (-0.5,0) -- (0,0);
    \draw[thick] (0,0) -- (2,0);
    \draw[thick] (2,0) -- (4,0);
    \draw[thick] (4,0) -- (5,0);
    \draw[thick] (5,0) -- (7,0);
    \draw[thick,->] (7,0) -- (7.5,0);
        \filldraw[black] (0,0) circle (2pt) node[anchor=west] {};
        \filldraw[black] (7,0) circle (2pt) node[anchor=east] {};

    % draw vertical lines
    \foreach \x in {0,1.05,2.1,3.15,3.85,4.9,5.95,7}
      \draw[thick,dotted] (\x cm,20pt) -- (\x cm,0pt);

    % draw nodes
    \draw (0,0) node[below=3pt] {$ 0\% $} node[above=6pt] { none \hspace{2mm}   a few };
    \draw (1,0) node[below=3pt] {$ 15\% $} node[above=6pt] {\hspace{12mm}some};
    \draw (2,0) node[below=3pt] {$ 30\% $} node[above=5pt] {\hspace{13mm}many};
    
    \draw (3,0) node[above=10pt] {\hspace{10mm}about};
    \draw (3,0) node[below=3pt] {$ 45\% $} node[above=1pt] {\hspace{10mm}half};
    
    \draw (4,0) node[below=3pt] {$ 55\% $} node[above=9pt] {\hspace{8mm}major};
    \draw (4,0) node[above=1pt] {\hspace{8mm}-ity};
    
    \draw (5,0) node[below=3pt] {$ 70\% $} node[above=6pt] {\hspace{8mm}most};
    
    \draw (6,0) node[below=3pt] {$ 85\% $} node[above=8pt] {\hspace{10mm}almost};
    \draw (6,0) node[above=1pt] {\hspace{10mm}all};
    
    \draw (7,0) node[below=3pt] {$ 100\% $} node[above=6pt] {\hspace{6mm}all};
  \end{tikzpicture}
\end{figure}

%reference: https://www.overleaf.com/learn/latex/LaTeX_Graphics_using_TikZ%3A_A_Tutorial_for_Beginners_(Part_1)%E2%80%94Basic_Drawing



==> tables/label_differences.tex <==
\begin{table*}
\caption{Android and iOS Privacy Label Differences (Just Dance Now)}
    \centering
    \label{tab:label_differences}
    \begin{tabular}{M{15mm}|M{75mm}|M{75mm} } 
    \Xhline{2.5\arrayrulewidth}
    Structure & Android Label & iOS Label\\
    \Xhline{2.5\arrayrulewidth}
    Privacy Labels & ``Data Safety'' & ``App Privacy''\\
    \hline
    Compact Label & \includegraphics[width=60mm]{figures/JDN_android_compact_april.png} & \includegraphics[width=65mm]{figures/JDN_compact_april.png}\\
    \hline
    Expanded Label & \includegraphics[width=70mm]{figures/expanded_diff1.png} & \includegraphics[width=72mm]{figures/expanded_diff2.png}\\
    \hline
    Data Collection Purposes & \includegraphics[width=70mm]{figures/location_purpose.png} & \includegraphics[width=70mm]{figures/app_func2.png}\\
    \hline
    Security Practices & \includegraphics[width=55mm]{figures/youtube_kids.png} & N/A\\
    \hline
    Privacy Policy & \includegraphics[width=60mm]{figures/android_learn_more.png} \includegraphics[width=60mm]{figures/android_privacy_policy.png} &\includegraphics[width=60mm]{figures/iOS_links.png} \\
    \Xhline{2.5\arrayrulewidth}
    
     
    \end{tabular}
        \begin{tablenotes}
          \small
          \item Most labels included in this \autoref{tab:label_differences} were screenshots taken from the app Just Dance Now in April 2023, and the Android label on the ``Security Pratices'' row was from YouTube Kids. Apps that are intended for children are required to adhere to Google's Play Families Policies Requirements, and failure to comply with these requirements may lead to the suspension or removal of the app~\cite{google}. The ``Expanded Label'' row shows only a portion of the entire expanded label. N/A means that the question does not have a label addressing it. The idea of the above table comes from~\cite{zhangprivacy}.
        \end{tablenotes}
\end{table*}

% we used screenshots from JDN , only child-friendly apps have security practices so xxxx was taken from this app "Committed to follow the Play Families Policy"
% look at the category for family apps
% include independent security review
